Unlocking the Power of Inline Floating-Point Operations on Programmable Switches

The advent of switches with programmable dataplanes has enabled the rapid development of new network functionality, as well as providing a platform for acceleration of a broad range of application-level functionality. However, existing switch hardware was not designed with application acceleration in mind, and thus applications requiring operations or datatypes not used in traditional network protocols must resort to expensive workarounds. Applications involving floating point data, including distributed training for machine learning and distributed query processing, are key examples. In this paper, we propose FPISA, a floating point representation designed to work efficiently in programmable switches. We first implement FPISA on an Intel Tofino switch, but find that it has limitations that impact throughput and accuracy. We then propose hardware changes to address these limitations based on the open-source Banzai switch architecture, and synthesize them in a 15-nm standard-cell library to demonstrate their feasibility. Finally, we use FPISA to implement accelerators for training for machine learning and for query processing, and evaluate their performance on a switch implementing our changes using emulation. We find that FPISA allows distributed training to use 25-75% fewer CPU cores and provide up to 85.9% better throughput in a CPU-constrained environment than SwitchML. For distributed query processing with floating point data, FPISA enables up to 2.7x better throughput than Spark.

==> char.tex <==
% !TEX root = paper.tex

==> discussion.tex <==
% % !TEX root = paper.tex
% \section{Advanced Floating point Operations}
% \label{sec:discussion}
% In this paper, we have covered the two commonly-used floating point operations -- addition and comparison.
% They are sufficient for many distributed applications.
% However, other more complex and costly floating point operations may be needed in the future with emerging applications (\eg, congestion control~\cite{xcp,rcp} and network security~\cite{10.1145/3230543.3230555}). 
% To pave the way for future PISA implementations, we briefly discuss the possibility of supporting them.

% \niparagraph{Mulplication and division.} 
% The flow of floating point multiplication is similar to that of addition in \secref{sec:add}.
% The two major differences are (1) the two exponents are added, and (2) the two mantissas are multiplied, all as integers.
% For small floating point types, the mantissa multiplication can be implemented as a table lookup, without hardware modifications.
% For larger floating point types, integer multiplers could be added to the hardware. We implement one based on Banzai and find its overhead is acceptable: approximately the same as an adder and a boolean module \wrt power and area. 
% %Hence, we expect that FP multiplication can be supported soon.
% %Hence, adding multipliers would be practical, but

% Floating point division has a different flow and takes more clock cycles than other basic operations~\cite{10.1145/243439.243481}, which means it is unsuitable to have a direct hardware implementation in programmable switches.
% For some use cases, division can be implemented by converting the dividend to its reciprocal at the end-host and then multiplying in the switch.



% \niparagraph{Logarithms.}
% % Based on the following formula
% % \begin{subequations}
% % 	\label{eq:log}
% % \begin{align*}
% %     log(x) &= log (2^{x_{exp}}\times x_{man})\\
% %           &= x_{exp} \times log(2) + log(x_{man})
% % \end{align*}
% % \end{subequations}
% The core operation of a floating point logarithm is the integer logarithm of the mantissa.
% As prior research~\cite{5470752,201474,10.1145/98267.98294} shows, this can be done by a lookup table of fewer than 2000 entries with low error (<1\%). 
% %Conceivably, PISA provides suitable table abstraction to fulfill this purpose.
% %The specific implementation depends on the error requirement and resource constraint.


% \niparagraph{Square roots.}
% Square roots are even more expensive and time-consuming (\eg, more than 20 clock cycles) than division~\cite{10.1145/243439.243481,762835,624623}.
% As with logarithms, we suggest a lookup-table-based approximation for this algorithm. 
% %The programmer should try to avoid moving this operation to the switch.  

==> implementation.tex <==
% !TEX root = paper.tex
\section{Implementation and Hardware Enhancements}
\label{sec:impl}


\iffalse
\niparagraph{More CPU-like pipeline.} To realize full-functional FP addition, rounding needs to be included. 
Also, it is better to adjust the in-memory exponent timely, instead deferring it until the aggregation is done. 
To achieve this, PISA's pipeline should be re-designed to support accessing any stage's memory from arbitrary stage and dependency detection. 
Apparently, such \textit{significant architectural change} runs counter to the principle of PISA (and even general networking data plane) and is also unnecessary for distributed training workload, let alone the design complexity and feasibility.   
\fi

==> motivation.tex <==
% !TEX root = paper.tex
\begin{comment}
\section{Motivation and Challenges}
\label{sec:mov}
\subsection{Why Running In-switch Aggregation on PISA?}
\label{sec:why}
There have been in-switch aggregation projects for distributed training on different platforms, including FPGA~\cite{10.1145/3307650.3322259} and fixed-functional ASIC~\cite{9138924,10.5555/3018058.3018059,adiga2002overview,sharpv2}.
Here we discuss their limitations and justify why it is better to run the same thing on PISA.

For FPGA, it is qualified as a proof-of-concept prototype. 
However, FPGA itself, maybe enough for SmartNIC, is not able to handle massive traffic like a commodity switch.  
For example, Xilinx's next-generation flagship FPGA can achieve at most 3.2Tbps~\cite{versal}, while Barefoot's Tofino2 can easily achieve 6.4Tbps and up tp 12.8Tbps~\cite{barefoot2}. 
Also, to achieve comparable performance, FPGA is much more expensive and consumes more human labor for design.
Hence, FPGA is not a good fit for real-world development and deployment.

Fixed-functional ASIC can achieve high performance with relative low cost.
Its drawback is mainly the inflexibility.
\Ie, it is typically tied to specific FP format, set of operations, and often protocol. 
For example, it takes Mellanox's SHARP four years (a generation) to evolve from small HPC reduction to large ML workload~\cite{10.5555/3018058.3018059,sharpv2}. 
Another example is FP format. 
Modern ML adopts multiple FP formats with various size to make the compute and data movement inexpensive, and thus facilitate the training procedure~\cite{micikevicius2017mixed,apex}. 
Moreover, new ML-specific formats (\eg, bfloat16~\cite{dean2012large,bfloat16,kalamkar2019study} and TF32~\cite{tf32}) are being invented and applied.
Apparently, fixed-functional ASIC cannot keep up with the evolution of FP formats (\ie, typically only regular single/double-precision formats are supported). 

Both FPGA and fixed-functional ASIC solutions require dedicated hardware units (\ie, off the regular switch data path) to perform in-switch aggregation, which themselves can become the potential bottleneck inside the switch. 


On the contrary, PISA achieves the best tradeoff between throughput (\eg, $32\sim64$ 100/400Gb ports) and flexibility (\eg, new numeric representations, applications, and protocols) on off-the-shelf switches. 
Also, all packet processing is inline (\ie, within the programmable pipeline) with good scalability, which does not incur extra overhead or bottleneck. 
Last but not least, other regular network tasks can still run on PISA simultaneously.

\end{comment}



\begin{comment}
\begin{itemize}[leftmargin=*]
\item Readily available, especially if we broaden the definition to
  include non-Barefoot programmable switches
\item Best tradeoff between throughput (32-64 100-400G ports) and
  flexibility (new numeric representations, applications, protocols,
  etc)
\item Doesn't require dedicated hardware, in the sense that the same
  switch can be used for aggregation and regular networking tasks;
  even the architectural resources don't have to be dedicated
\item Why not a fixed-function FPU like SHARP? Tied to a specific
  floating point representation, set of operations, and often
  protocol. Example: going from small HPC reductions to large ML
  workloads required a new hardware generation (SHARP v2) and around 4
  years
\item Why not a FPGA? Even more flexibility, but achieving the same
  throughput level is going to be expensive or impossible 
\end{itemize}
\end{comment}

